Physics-Informed Neural Network for Parameter Identification: a Buck Converter Case Study

System-level condition monitoring methods estimate the electrical parameters of multiple components in a converter to assess their health status. The estimation accuracy and variation can differ significantly across parameters. For instance, inductance estimations are generally more accurate and stable than inductor resistance in a buck converter. However, these performance differences remain to be analyzed with a more systematic approach otherwise the condition monitoring results can be unreliable. Therefore, this paper analyzes the training loss landscape against multiple parameters of a buck converter to provide a systematic explanation of different performances. If the training loss is high and smooth, the estimated circuit parameter typically is accurate and has low variation. Furthermore, a novel physics-informed neural network (PINN) is proposed, offering faster convergence and lower computation requirements compared to an existing PINN method. The proposed method is validated through simulations, where the loss landscape identifies the unreliable parameter estimations, and the PINN can estimate the remaining parameters.

==> section/3_0problemanalysis.tex <==
% 1. 这一章节对我们构建的方法进行分析。总而言之，这个优化问题是个多参数，非线性，非凸的病态问题。这个章节会尝试着解释这些性质并进行定量分析。
% 2. 特性分析
% 3. 误差曲线展示和比较

This section analyzes the characteristics of the proposed method from the optimization perspective. The equivalent optimization problem can be written as \eqref{equivalent_opt_problem}, searching for the optimal $\hat {\theta}_0$ to minimize the loss.
\begin{equation}
     \arg\min_{\hat {\theta}_0} Loss(\hat {\theta}_0)
     \label{equivalent_opt_problem}
\end{equation}
It is a nonlinear, high-dimensional [xx], non-convex, and ill-conditioned optimization problem. These characteristics are analyzed in the following sections. Because of these characteristics, the proposed method only monitors $\hat{\theta}_1$ that has a stronger effect on the loss. 

The characteristics are independent of the optimizer and only depend on the loss function, so the analysis also works for methods in [xx-xx] since the optimization problem is formed similarly.

\subsection{Nonlinearity}
The nonlinearity comes from the physics model, which involves the state-space model and Forward Euler method solving time-domain equations. On the one hand, the physics model sets the constraints of the parameters and reduces the solution space [xx]. On the other hand, it causes nonlinearity and can increase the computation burden [xx]. 
\subsection{Non-convex}
The non-convex comes from the analysis of the Hessian matrix of the loss function, which is non-positive definite [xx], indicating the existence of the local minimal that can trap the optimizer and lead to errors in estimations.
\subsection{Ill-conditioned}
The optimization problem includes multiple parameters, and each of them affects the state vector in different ways, e.g., the inductance $L$ can change the phase of the current and the peak-to-peak ripple size, while the on-state resistance ($R_\mathrm{dson}$) can only slightly change the mean value of the current and voltage \cite{She2024}. 

These effects can be quantified by the condition number [xx]. The equation is xxx. If the condition number is close to one, the effects from different variables are on a similar scale and the problem tends to be easier to solve. However, the condition number of the proposed method is much greater than one, meaning that some of the parameters are difficult to solve. %, 


Equation 1: dE/dtheta
Equation 2：dE^2/dtheta^2




%The 


% This section analyzes the loss landscape and quantifies the difficulties of multiple parameter estimations in system-level condition monitoring. 

% The loss function built in the above section involves the state-space model and Forward Euler method, making the optimization method highly nonlinear. Additionally, the challenge lies in the multiple parameters affecting the state vector differently, e.g., the inductance $L$ can change the phase of the current and the peak-to-peak ripple size, while the on-state resistance ($R_\mathrm{dson}$) can only slightly change the mean value of the current and voltage \cite{She2024}. 




% This section analyzes the condition number of the parameter estimation problem, the condition number can be calculated using the xxx.

% Equation 1: dE/dtheta
% Equation 2：dE^2/dtheta^2

% With certain noise levels/ADC resolution/delay? Put a figure here, showing that the optimization surface becomes flat so the parameter cannot be identified anymore.



% This section analyzes the difficulty in estimating different parameters. 

% 1. Why some of the parameters are difficult to estimate. 
% 2. Reason: parameters are smaller and have less impact on the state vector.
% 3. Quantify the impact by doing sensitivity analysis and condition number 
% List equations from loss E to theta0, and then from loss E^2 to theta0.
% 4. Results (in the validation section): the curve of sensitivity? A table comparing the condition number. 
% 5. Discussion about these two terms: the sensitivity shows the difference of xxx, in which theta1 is much higher than theta2. Condition number wise, theta1 is greater than theta2 in multiple scales, showing the 

% Try to add some noises and show the curvate dispears...



==> section/4_0CharacteristicValidation.tex <==


This section uses a buck converter (parameters are listed in Table~\ref{tab_circuit_param}) to demonstrate the characteristics of the optimization problem. 

\subsection{Nonconvex}
The Hessian matrix and the eigenvalues.


The loss landscape is visualized in Fig. xxx in the ideal condition without including noise, delay, or analog-digital conversions. Even in such an ideal condition, the loss landscape of each parameter varies in a great range. The $\theta_0 = \{ L, C,R \}$ is much higher than the other parameters. Parameters $R_\mathrm{C}$, $R_\mathrm{dson}$ have a shallower curve and a lot of oscillations which can trap the optimizer into local optimal solutions. The most challenging one is the diode forward voltage, as it does not show the converging trend towards the actual value, leading to a wrong estimation.

\subsection{Condition Number}
The condition numbers of the estimated parameters are calculated and listed in Table~\ref{tab_condition_number}. It is worth noting that the condition number can only reflect the second-order derivative of a certain point at the loss landscape, it can only show the curvature relationship at a certain place. The optimal point and some more deviation points are selected to further demonstrate the quantify 



% Give a table, listed all condition numbers of the variables. 



